Learning on Manifolds: Universal Approximations Properties using Geometric Controllability Conditions for Neural ODEs

In numerous robotics and mechanical engineering applications, among others, data is often constrained on smooth manifolds due to the presence of rotational degrees of freedom. Common datadriven and learning-based methods such as neural ordinary differential equations (ODEs), however, typically fail to satisfy these manifold constraints and perform poorly for these applications. To address this shortcoming, in this paper we study a class of neural ordinary differential equations that, by design, leave a given manifold invariant, and characterize their properties by leveraging the controllability properties of control affine systems. In particular, using a result due to Agrachev and Caponigro on approximating diffeomorphisms with flows of feedback control systems, we show that any map that can be represented as the flow of a manifold-constrained dynamical system can also be approximated using the flow of manifold-constrained neural ODE, whenever a certain controllability condition is satisfied. Additionally, we show that this universal approximation property holds when the neural ODE has limited width in each layer, thus leveraging the depth of network instead for approximation. We verify our theoretical findings using numerical experiments on PyTorch for the manifolds S2 and the 3-dimensional orthogonal group SO(3), which are model manifolds for mechanical systems such as spacecrafts and satellites. We also compare the performance of the manifold invariant neural ODE with classical neural ODEs that ignore the manifold invariant properties and show the superiority of our approach in terms of accuracy and sample complexity.

==> Comments.tex <==
Weaknesses

[W1] Outside of simple and known manifolds, Assumption is very difficult to satisfy in practice. The authors could explain how the deal with unknown manifolds, and what are the implications of an imperfect manifold.

Minor Comments

[C1] The definition of ball in 2. Notation has a typo. Instead of r, it should be y. The locally Lipschitz definition also has a typo, if the condition is satisfied for all x,y, then the ball should be around z. In other words, x cannot be used twice.

Done


[C2] Section 4 is the only part of the paper which requires some re-writing.

    After Theorem 4, the text immediately makes reference to Theorem 5, which has not been presented yet.
    In Theorem 5, X needs to be defined.
    In the proof of Theorem 5, a reference to Proposition 6 is made. This proposition has not been introduced. I suggest the authors move this proof to the Appendix where Proposition 6 is.

    Done

[C3] The authors should be more precise about their citations. The authors say: "This follows from Lee(2013)", this great book has over 400 pages, the Theorem or at least chapter of the book needs to be provided. 

==> Neural ODE on Sphere/Comments.tex <==
Weaknesses

[W1] Outside of simple and known manifolds, Assumption is very difficult to satisfy in practice. The authors could explain how the deal with unknown manifolds, and what are the implications of an imperfect manifold.

Minor Comments

[C1] The definition of ball in 2. Notation has a typo. Instead of r, it should be y. The locally Lipschitz definition also has a typo, if the condition is satisfied for all x,y, then the ball should be around z. In other words, x cannot be used twice.

Done


[C2] Section 4 is the only part of the paper which requires some re-writing.

    After Theorem 4, the text immediately makes reference to Theorem 5, which has not been presented yet.
    In Theorem 5, X needs to be defined.
    In the proof of Theorem 5, a reference to Proposition 6 is made. This proposition has not been introduced. I suggest the authors move this proof to the Appendix where Proposition 6 is.

    Done

[C3] The authors should be more precise about their citations. The authors say: "This follows from Lee(2013)", this great book has over 400 pages, the Theorem or at least chapter of the book needs to be provided. 
